Sparse Hierarchical Tucker Factorization and its Application to Healthcare

We propose a new tensor factorization method, called the Sparse Hierarchical-Tucker (Sparse H-Tucker), for sparse and high-order data tensors. Sparse H-Tucker is inspired by its namesake, the classical Hierarchical Tucker method, which aims to compute a tree-structured factorization of an input data set that may be readily interpreted by a domain expert. However, Sparse H-Tucker uses a nested sampling technique to overcome a key scalability problem in Hierarchical Tucker, which is the creation of an unwieldy intermediate dense core tensor; the result of our approach is a faster, more space-efficient, and more accurate method. We extensively test our method on a real healthcare dataset, which is collected from 30K patients and results in an 18th order sparse data tensor. Unlike competing methods, Sparse H-Tucker can analyze the full data set on a single multi-threaded machine. It can also do so more accurately and in less time than the state-of-the-art: on a 12th order subset of the input data, Sparse H-Tucker is 18x more accurate and 7.5x faster than a previously state-of-the-art method. Even for analyzing low order tensors (e.g., 4-order), our method requires close to an order of magnitude less time and over two orders of magnitude less memory, as compared to traditional tensor factorization methods such as CP and Tucker. Moreover, we observe that Sparse H-Tucker scales nearly linearly in the number of non-zero tensor elements. The resulting model also provides an interpretable disease hierarchy, which is confirmed by a clinical expert.

==> content/baseline.tex <==
\subsubsection{Hierarchical Tucker and its Limitations}
\noindent\textbf{Model}\label{sec:Htuckermodel}
Our baseline model is the Hierarchical Tucker (H-Tucker in short) format
presented in~\cite{Grasedyck2010}.
Its main intuition of draws on the recursive splitting of the tensor
modes, resulting in a binary tree (called \textit{dimension tree} $\mathcal{T_I}$). Each node
of this tree contains a subset $t \subset \{1, \dots,
d \}$ of the modes and is either a leaf and singleton
$t={\mu}$ or the union of its two disjoint successors $t_1, t_2: t = t_1 \cup t_2 $.
The model also receives a target rank $(k_t)_{t \in \mathcal{T_I}}$ as input,
which governs the approximation error of the decomposed tensor. The model's output factors
are the following: $(\T{B}_t)_{t \in \mathcal{I}(T_I)} \in
 \mathbb{R}^{k_t \times	k_{t_1} \times k_{t_2}}, (\M{U}_{t})_{t \in \mathcal{L}(T_I)}
\in \mathbb{R}^{I_t \times k_t}$, where $\{t_1, t_2\} = s(t)$.
The notation indicates that there exist $\M{U}_t$ matrices corresponding
to the leaves of the tree and $\T{B}_t$ tensors (called transfer tensors hereafter)
corresponding to the interior nodes.
$s(t)$ denotes the set of successor nodes of node $t$.
Since the rank of the root node is equal to $1$ ($k_{t_r}=1$),
the factor $\T{B}_{t_r}$ is a matrix. An example of this model in tensor network notation
is given in Figure~\ref{fig:htucker_pure}.


%The goal goal is to approximate a high-order tensor as an hierarchy of low-order tensors
%(in particular, 2nd and 3rd order). 
%For example, if the resulting hierarchy is a balanced tree, the target model  $\mathcal{T_I}$ for
%an $4$-order input tensor will be approximated as in  where the leaves are denoted by $\mathcal{L(T_I)}$
%(2nd order tensors)  and the internal nodes are denoted by $\mathcal{I(T_I)}$ (3rd order tensors).
%The root node of the tree  $t_r$ is a matrix.

\begin{figure}
	\centering
	\includegraphics[scale=0.25]{figures/htucker_pure}
	\caption{Hierarchical Tucker format in tensor
		network notation (4-order tensor, balanced dimension tree).}
	\label{fig:htucker_pure}
\end{figure}


\noindent\textbf{Re-construction of a tensor via the model's factors} The
matricization $\T{A}^{(t)}$ corresponding to the subset $t$ combines all modes
contained in $t$ in row indices and the rest of the modes into column indices.
If $\{t_1, t_2\} = s(t)$, then the \textit{nestedness property} dictates that given
any bases $\M{U}_t \in \mathbb{R}^{(I_{t1}I_{t2}) \times k_t}, \M{U}_{t_1}
\in \mathbb{R}^{I_{t_1} \times k_{t_1}},
\M{U}_{t_2} \in \mathbb{R}^{I_{t_2} \times k_{t_2}}$ for
the column spaces of $\T{A}^{(t)}$, $\T{A}^{(t_1)}$, $\T{A}^{(t_2)}$,
there exists a tensor $\T{B}_t \in \mathbb{R}^{k_t \times
	k_{t_1} \times k_{t_2}}$ of coefficients for the representation of
the columns of $\M{U}_t$ through the columns of $\M{U}_{t_1}, \M{U}_{t_2}$:
\begin{equation}
(\M{U}_t)_i = \sum_{j=1}^{k_{t_1}} \sum_{l=1}^{k_{t_2}}
(\T{B}_t)_{i, j , l} \left( (\M{U}_{t_1})_j \otimes (\M{U}_{t_2})_l \right)
\label{eq:nestedness}
\end{equation}

%In Figure~\ref{fig:tranfer},
%we illustrate its form before the execution of Equation~\ref{eq:nestedness},
%as well as its final form after its execution and the reshaping operation
%required to turn the tensor into a matrix.

%\begin{figure}
%	\centering
%	\includegraphics[scale=0.3]{figures/transfer_tensor}
%	\caption{Transfer tensor and its final form after the necessary reshaping operation. TODO: change to 4-order and put all the notations}
%	\label{fig:tranfer}
%\end{figure}

Equation~\ref{eq:nestedness} implies that it is sufficient
to provide the transfer tensors  $(\T{B}_t)_{t \in \mathcal{I}(T_I)}$
and the matrices $(\M{U}_{t})_{t \in \mathcal{L}(T_I)}$, in order to
re-construct $(\M{U}_{t})_{t  \in \mathcal{I}(T_I)}$.
If the nestedness property holds, the representation
$(\T{B}_t)_{t \in \mathcal{I}(T_I)},
(\M{U}_{t})_{t \in \mathcal{L}(T_I)}$
is an H-Tucker representation~\cite{Grasedyck2010}.
Given that we have re-constructed the matrices $\M{U}_t,
t \in \{t_1, t_2\} = s\{t_r\}$, corresponding to the second level
of the tree, the final input tensor approximation is given in
vectorized form as follows:
\begin{equation}
vec(A) \approx \sum_{j=1}^{k_{t_1}} \sum_{l=1}^{k_{t_2}}
(\M{B}_{t_r})_{j , l} \left( (\M{U}_{t_1})_j \otimes (\M{U}_{t_2})_l \right)
\label{eq:reconstruct}
\end{equation}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.25]{figures/htucker_expl2}
	\caption{Step-by-step representation of Algorithm~\ref{alg:htucker_base}
		in tensor network notation. We assume a $4$-order tensor and a balanced
		dimension tree, as the one shown in Figure~\ref{fig:htucker_pure}.
		Note that the tensor $\T{C}_1$ originates from Line 6, where it is initialized by  $\T{C}_2$.
		The steps corresponding to Lines 8-11 are illustrated for a single iteration (construction of
		tensor $\T{B}_{I_1}$) and update of core tensor.}
	\label{fig:ht_story}
\end{figure}

\begin{algorithm}[t]
	\begin{algorithmic}[1]
		\Require Input tensor $\T{A} \in \mathbb{R}^I$, tree
		$\mathcal{T_I}$ (depth $p>0$), target rank $(k_t)_{t \in \mathcal{T_I}}$
		\Ensure $(\T{B}_t)_{t \in \mathcal{I}(T_I)}, (\M{U}_{t})_{t \in \mathcal{L}(T_I)}$
		\For{ each singleton $t \in \mathcal{L(T_I)}$}
		\State $\M{U}_{t} \gets k_t$ left leading singular vectors
		of $\T{A}^{(t)}$ \label{htucker:line2}
		\EndFor
		\State Compute core tensor: $\T{C}_p := (\M{U}^T_1, \dots, \M{U}^T_d)  \circ \T{A} $
		\For{ $l = p-1, \dots, 1$ } 
		\State $\T{C}_l := \T{C}_{l+1}$
		\For{ each node $t \in \mathcal{I(T_I)}$ on level $l$}
		\State $\M{U}_{t} \gets k_t$ left leading singular vectors of $(C_{l+1})^{(t)}$
		\State $\{ t_1, t_2 \} := s(t)$
		%\State $(\T{B}_t)_{i,j,v} := < (\M{U}_t)_i,  (\M{U}_{t_1})_j \otimes
		%(\M{U}_{t_2})_v  > $ \label{htucker:line9}
		\State $\T{B}_t \gets$ reshape $ \M{U}^T_t : \mathbb{R}^{k_t \times
			k_{t_1}  k_{t_2}}  \rightarrow \mathbb{R}^{k_t \times
			k_{t_1} \times k_{t_2}}$
		\State Update core tensor: $\T{C}_l := \M{U}^T_t  \circ \T{C}_l $
		\EndFor
		\EndFor
	    \State $\{ t_1, t_2 \} := s(t_r)$
		%\State $\T{B}_{t_r} \gets$ reshape $ \M{U}^T_t : \mathbb{R}^{k_t \times
		%	k_{t_1}  k_{t_2}}  \rightarrow \mathbb{R}^{k_t \times
		%	k_{t_1} \times k_{t_2}}$
		\State $\T{B}_{t_r} \gets \T{C}_1$ \Comment{store as a $\mathbb{R}^{k_{t_1} \times  k_{t_2}}$ matrix}
	\end{algorithmic}
	\caption{Hierarchical Tucker factorization~\cite{Grasedyck2010} }
	\label{alg:htucker_base}
\end{algorithm}



\noindent\textbf{Factorization algorithm} \label{sec:shtucker_svd}

% Another closely related
%method (Tensor Train mode), belonging to the tensor network family as well,
%was developed in~\cite{Oseledets2011}, in which the dimension tree is a line graph.

%There are several issues limiting the scalability of the above
%method. 
%%At first, there is a technical issue that limits
%%the practicability of Algorithm~\ref{alg:htucker_base},
%%as concerns its implementation on
%%the most widely acclaimed mathematical toolbox (Matlab).
%In particular, the matricization of a high-order tensor into a matrix
%is limited by the maximum size of a sparse matrix.
%As such, the formation of the necessary reshapings
%in order to extract their leading
%left singular vectors becomes easily intractable
%as the tensor order grows.
%
%As an example, consider the
%case of unfolding a sparse d-order tensor
%$\T{A} \in \mathbb{R}^{n^d}$. %, where   $n_{t} = I, \forall t \in\{1, \dots , d\}$  w.r.t.~a leaf node.
%The leading singular vector computation requires
%the construction of a sparse $n^{d-1} \times n$
%matrix $\M{T} = {\T{A}^{(t)}}^T$ and the eigendecomposition of
%the product $\M{T}^T \M{T}$. However,
%matrix  $ \M{T}$ cannot be formed on a server with 128GB RAM
%even for $n=100$ and $d=20$.
%
%\comment{The way we formulated the above argument in the submitted
%	version may be misleading. The "128GB RAM" point may lead someone to believe
%	that the problem is related to lack of memory. Instead, due to the column-wise
%	format of storing sparse matrices, the storage of an $n^{d-1} \times n$ sparse
%	is trivial \textit{ unless $n^{d-1} > $ MAXSIZE of Matlab}, i.e.~ the maximum
%	size supported from Matlab for sparse matrices. We have to correct this argument
%	in the future.
%	
%	The memory problem argument would be suitable here, if both row and column
%	index sets were huge. Thus, it would apply to the next section for
%	the leverage scores' extraction. }
%
%In order to overcome this issue, we exploit the
%following observation:
%\begin{remark}
%	Let $I^{(t)}_{nz} \subseteq I^{(t)}$ be the set of indices of non-zero rows
%	of $\M{T} = {\T{A}^{(t)}}^T$ following their original ordering. Then:
%	\[ \M{T}(I^{(t)}_{nz}, :)^T \M{T}(I^{(t)}_{nz}, :) =
%	\M{T}^T \M{T} \]
%\end{remark}
%
%Following the above observation, we can efficiently extract
%the leading left singular vectors of each one of the leaf unfoldings.

The method for computing
the H-Tucker format of a tensor is provided
in Algorithm~\ref{alg:htucker_base}~\cite{Grasedyck2010}.
The pseudocode follows the presentation in~\cite{kressner2012htucker},
which is closer to how the algorithm is implemented in practice.
Figure~\ref{fig:ht_story} provides a step-by-step illustration
of the algorithm, in tensor network notation. Notice how
this formalism facilitates explanation and algorithmic modeling of tensors.
At first, the algorithm iterates over all leaf nodes $t$ and computes
the left singular vectors of each $t$-mode matricization $\T{A}^{(t)}$.
In Line 4, the computed bases of tensor unfoldings are
multi-linearly multiplied by the input tensor.
The resulting core tensor $\T{C} $ is further reshaped w.r.t.~the
row modes of each one of the interior nodes and the left singular
vectors of this matrix are computed. By reshaping $ \M{U}^T_t $
 to a $\mathbb{R}^{k_t \times 	k_{t_1} \times k_{t_2}}$ tensor,
we acquire the transfer tensor $\T{B}_t$.
After having iterated through all levels but the one containing the root,
the only two non-singleton modes of the core tensor $\T{C}$
are the ranks corresponding to the root node's successors. This
means that if $\{ t_1, t_2 \} := s(t_r)$, then $\T{B}_{t_r}$ can be considered
as a matrix of size $k_{t_1} \times k_{t_2}$.


\noindent\textbf{Limitations} The method described suffers from
severe scalability issues as the tensor order increases.
Despite the fact that the final form of H-Tucker
($(\T{B}_t)_{t \in \mathcal{I}(T_I)},
(\M{U}_{t})_{t \in \mathcal{L}(T_I)}$)
requires linear storage to the tensor order $d$, the
core tensor computed in Line 4 is in general
both \textit{dense} and \textit{high-order}.
Its size ($\prod_{t \in \mathcal{L}(T_I)} k_t $) grows
\textit{exponentially} to the order of the input tensor.
As a result, this method faces
a potential \textit{memory blow-up} as it requires further decomposing an
\textit{intermediate result} that may not even fit into memory.
It is worth stressing out that this is expected to happen even
if the input tensor is sparse, since its multi-linear multiplication
with the dense leading left singular vectors of the leaf unfoldings
will generally produce a dense intermediate result.

%The Hierarchical Tucker model provided by the method described above
%is shown in tensor network notation in Figure~\ref{fig:ht_dense}.


==> content/related_work.tex <==
\section{Related Work} \label{sec:related}


%
%Targeting a different problem of tensor completion
%for compressive sensing, the work in~\cite{Da2013} 

%	\begin{itemize}
%		\item ~\cite{Phan2013}
%	
%		\item ~\cite{Kang2012}
%		
%		\item ~\cite{Zhou2014}: Very recent work dealing with high individual mode sizes,
%		but not very high dimensional tensors
%		
%		\item ~\cite{Fang2014}
%		
%		\item ~\cite{Kolda2008}
%	
%		
%		\item ~\cite{Sidiropoulos2014}: focuses on CP tensors
%		
%
%	\end{itemize}
	
%	\item Our tensor sketching approach could also be utilized as a
%	streaming tensor analysis method~\cite{Sun2006, Jiang2014}. Comparison. Error bounds?
%	FEMA: no parallelization potential (sketching sketches), 
%	% unable to handle
%	% higher-order tensors (cases when computations on tensor reshapings
%	% face memory or arithmetic limitations)
%	
%	\item Streaming Anomaly Detection Using Online Matrix Sketching: 
%	http://www.cse.psu.edu/~kasivisw/Adems.pdf

%		\item As also being pointed out in~\cite{Kuo2014}, imposing sparsity constraints
%		on high-dimensional tensors would involve a time-consuming parameter tweaking
%		for each one of the factor matrices. Instead, in this work, we propose a scalable version
%		of a tensor format that inherently produces compressed representations that do not
%		suffer from the curse of dimensionality.

==> figures/tikz_TN.tex <==
\begin{tikzpicture}[>=latex,scale=1.3]
\shade[ball color=mycyan!100!] (4,0) coordinate(Hm) circle (.9) ;
\end{tikzpicture}
\begin{tikzpicture}[>=latex,scale=1.3]
\shade[ball color=gray!10!] (4,0) coordinate(Hm) circle (.9) ;
\end{tikzpicture}
